Coupled Neural Associative Memories

We propose a novel architecture to design a neural associative memory that is capable of learning a large number of patterns and recalling them later in presence of noise. It is based on dividing the neurons into local clusters and parallel plains, very similar to the architecture of the visual cortex of macaque brain. The common features of our proposed architecture with those of spatially-coupled codes enable us to show that the performance of such networks in eliminating noise is drastically better than the previous approaches while maintaining the ability of learning an exponentially large number of patterns. Previous work either failed in providing good performance during the recall phase or in offering large pattern retrieval (storage) capacities. We also present computational experiments that lend additional support to the theoretical analysis.

==> Exponential_capacity_proof.tex <==
\section{Pattern Retrieval Capacity}\label{section_capacity}
In this section, we prove that the number of patterns that can be memorize by the proposed scheme is exponential in $n$, the pattern size. To this end, note that the number of patterns that can be memorized is only related to the size of the subspace that sub-patterns come from. In other words, the number of patterns $\mc{C}$ which the network memorizes does not depend on the learning or recall algorithms (except its obvious effect on the running time). Therefore, in order to prove that $\mc{C}$ could exponentially scale with $n$, we show there exists such a subspace with exponentially large number of members (in terms of $n$).


\begin{theorem}\label{theorem_exponential_solution}
Let $\mc{X}$ be the $\mc{C} \times n$ dataset matrix, formed by $\mc{C}$ vectors of length $n$ with entries from the set $\mc{S}$. Let also $k = rn$ for some $0<r<1$. Then, there exists a set of patterns for which $\mc{C} = a^{rn}$, with $a > 1$, and $\hbox{\text{rank}}(\mc{X}) = k <n$.
\end{theorem}

As a practical example, one could select $G$ and $u$ to have $0/1$ entries (i.e. $\gamma = \upsilon = 2$) and in $G$, $d^* = 10$. Then it is sufficient to have $S\geq 11$ to have a pattern retrieval capacity of $\mc{C} = 2^{rn}$. 

Finally, note that inequality (\ref{capaci_inequal}) corresponds to the worst-case scenario in constructing the patterns in the sense even if not all the patterns $\textbf{x} = \textbf{u}\cdot G$ satisfy the bound on maximum value of entries, still a polynomially many of them satisfy this requirement. These vectors correspond to the message vectors $\textbf{u}$ that are "sparse" as well, i.e. do not have all entries greater than zero. In this case, although one will not achieve the exponential scaling, it is possible to reach polynomial capacities which is still much better than the linear scaling in Hopfield networks \cite{hopfield}.



==> Recall_Algorithm_technical.tex <==
%\subsection{The Proposed Algorithm}
In this section, we briefly discuss our approach for addressing the aforementioned phases.
 
\textbf{Learning phase:} As we mentioned earlier, for the learning phase we use the learning algorithm proposed in \cite{KSS_ICML2013}. In the remaining, we  effectively assume that the connectivity matrices $W^{(\ell,d)}$ are known and satisfy Eq.~\ref{eq:orthogonal}. 

\textbf{Recall phase:} The proposed recall algorithm in this paper is the extension of the one  proposed in \cite{SK_ISIT2012} to the coupled neural networks. For the sake of completeness, we have summarized this approach in Algorithm \ref{algo:correction}, the goal of which is to correct (at least) a single error in a cluster with high probability. Let us remind ourselves of the performance of Algorithm~\ref{algo:correction}.

\begin{theorem}\label{theorem:isit}\cite{SK_ISIT2012}
When $\varphi \rightarrow 1$, Algorithm~\ref{algo:correction} can correct a single error in each cluster with probability at least $1- (\bar{d}/m)^{d_{\min}}$, where $\bar{d}$ and $d_{\min}$ are the average and minimum degree of the pattern nodes within the cluster domain.
\end{theorem}

We apply Algorithm \ref{algo:correction} \emph{sequentially} to neural clusters and neural planes as follows. We start with the first cluster in the first plane and apply Algorithm~\ref{algo:correction}. Once finished, we check the final state of the constraint nodes, expecting them to be all zero. 
% if all errors within the cluster have been corrected (simply by checking the final state of the constraint nodes, expecting to be all zero). 
% 
If not, we revert the values of the pattern nodes  to their initial values. We then proceed to the second cluster in the first plane and continue until we reach the last cluster in the last plane. We repeat the above sequential scheduling $t_{\max}$ times (see Algorithm~\ref{algo:coupled}). Repeating is particularly helpful since errors get corrected in each round which makes noisy clusters experience less amount of noise for the following rounds and thus higher success rate for the application of Algorithm~\ref{algo:correction} on the clusters. Note that by Theorem~\ref{theorem:isit}, Algorithm~\ref{algo:correction} can only guarantee the correction of a single error. Hence, applying Algorithm~\ref{algo:correction} to clusters with two or more errors might be unsuccessful. By sweeping $t_{\max}$ times over the clusters and planes, we try to correct noisy neurons one by one.  

%We apply Algorithm \ref{algo:correction} \emph{sequentially} to the neural planes in Figure~\ref{fig:coupled_model}, i.e., first we eliminate noise in the first plane, then the second one and so on. Once we have iterated over all planes, we go back and repeat this process as long as necessary.
%
%Within each plane, we apply a sequential scheduling again. More specifically, we apply Algorithm \ref{algo:correction} to the first neural cluster. Once finished, we check if all errors within the cluster have been corrected simply by checking the final state of the constraint nodes, expecting to be all zero. If not, we revert the values of the pattern nodes in that cluster to their initial values (before applying error correction). We then proceed to the next cluster until all clusters within the neural plane are covered. We repeat this process by going back to the first cluster as many times as necessary. Repeating this process will be helpful since some of the errors might have been corrected in the previous round, resulting in clusters that had two or more errors in their domain ending up with only a single error in this iteration. Therefore, they can correct this error now, helping their neighboring clusters. Algorithm~\ref{algo:coupled} summarizes the proposed algorithm.
\begin{algorithm}[t]
\caption{Error Correction Within Cluster \cite{SK_ISIT2012}}
%Finding Target with Entropy plus the logarithm of the diameter of the constraint graph Search Queries}
\label{algo:correction}
\begin{algorithmic}[1]
\REQUIRE{Connectivity matrix $W^{(\ell,d)}$, threshold $\varphi$, iteration $t_{\max}$.}
\ENSURE{Correct memorized sub-pattern $\textbf{x}^{(\ell,d)}$.}
% =[x^{(\ell,d)}_1,\dots,x^{(\ell,d)}_{n_{\ell,d}}]$}
\FOR{$t = 1 \to t_{\max}$} 
\STATE \textit{Forward iteration:} Calculate the weighted input sum $ h_i = \sum_{j=1}^n W^{(\ell,d)}_{ij} x^{(\ell,d)}_j,$ for each neuron $y^{(\ell,d)}_i$ and set:
\[ y^{(\ell,d)}_i = \left\{
\begin{array}{cc}
1, & h_i < 0\\
0, & h_i = 0\\
-1, & \hbox{otherwise}
\end{array} \right. 
\]
\STATE \textit{Backward iteration:} Each neuron $x^{(\ell,d)}_j$ computes
\[ g^{(\ell,d)}_j = \frac{\sum_{i=1}^{m_{\ell,d}} W^{(\ell,d)}_{ij} y^{(\ell,d)}_i }{\sum_{i = 1}^{m_{\ell,d}}|W^{(\ell,d)}_{ij}|}. \]
\STATE Update the state of each pattern neuron $j$ according to $x^{(\ell,d)}_j = x^{(\ell,d)}_j + \hbox{sgn}(g^{(\ell,d)}_j)$
only if $|g^{(\ell,d)}_j| > \varphi$.
% \STATE $t \gets t + 1$
\ENDFOR
\end{algorithmic}
\end{algorithm}
%??? Take care of the footnote in ALGO
%\begin{minipage}{.48\textwidth}
\begin{algorithm}[t]
\caption{Error Correction of the Coupled Network}
%Finding Target with Entropy plus the logarithm of the diameter of the constraint graph Search Queries}
\label{algo:coupled}
\begin{algorithmic}[1]
\REQUIRE{Connectivity matrix ($W^{(\ell,d)},\forall \ell,\forall d$), iteration $t_{\max}$}
\ENSURE{Correct memorized pattern $\textbf{x} =[x_1,x_2,\dots,x_{n}]$}
\FOR{$t = 1 \to t_{\max}$} 
\FOR{$\ell = 1 \to L$} 
\FOR{$d = 1 \to D$}
\STATE Apply Algorithm~\ref{algo:correction} to  cluster $d$ of neural plane $\ell$.
\STATE Update the value of pattern nodes $\textbf{x}^{(\ell,d)}$ only if all the constraints in the clustered are satisfied. 
%\STATE $i \gets i + 1$
\ENDFOR
%\STATE $\ell \gets \ell + 1$
%\footnote{Note that we can stay in the loop several time for each plane and move to the next plane only after we are fully done with the current one.}
\ENDFOR 
%\STATE $t \gets t + 1$
\ENDFOR
\end{algorithmic}
\end{algorithm}
%\end{minipage}
\vspace{0.15cm}

We consider two variants of the above error correction algorithm. In the first one, called  \emph{constrained} coupled neural error correction, we provide the network with some side information during the recall phase. This is equivalent to "freezing" a few of the pattern neurons to known correct states, similar to  spatially-coupled  codes  \cite{kudekar}, \cite{pfister_istc}. In the case of neural associative memory, the side information can come from the context. For instance, when trying to fill in the blank in the sentence "The \emph{$\_$ at} flies", we can use the side information (flying) to guess the correct answer among multiple choices. Without this side information, we cannot tell if \emph{$\_$ at} corresponds to \emph{bat} or \emph{cat}.

In the other variant,  called \emph{unconstrained} coupled neural error correction, we perform the error correction without providing any side information. This is similar to many standard recall algorithms in neural networks and serves as a benchmark to compare our method with those of other work \cite{KSS}, \cite{SK_ISIT2012}.


Let $z^{(\ell)}(t)$ denote the \emph{average} probability of error for pattern nodes across neural plane $\ell$ in iteration $t$. A super constraint node in plane $\ell$ receives noisy messages from its neighbors with an average probability of $\bar{z}^{(\ell)}$, where 
$$\bar{z}^{(\ell)} = \frac{1}{2\Omega+1}\sum_{j=-\Omega}^{\Omega} z^{(\ell-j)} ~ \text{s.t.}~ z^{(l)} = 0,~\forall l\notin \{1,\dots,L\}.$$ In the following, we derive a recursive expression for $z^{(\ell)}(t)$ (all the proofs are provided in the Appendix). 
\begin{lemma}\label{lem:recursive}
Let us define $g(z)=1-\rho(1-z)+z\rho'(1-z)$ and $f(z;p_e) = p_e \lambda(z)$ . Then,
\beq \label{z_ell}
z^{(\ell)}(t+1) = f\left(\frac{1}{2\Omega + 1}\sum_{i=-\Omega}^{\Omega}g(\bar{z}^{(\ell-i)}(t);p_e\right).
\eeq
\end{lemma}
%with $z^{(i)} = 0$ for $i \leq 0$ and $i > L$. 
 The decoding  will be successful if $z^{(\ell)}(t+1) < z^{(\ell)}(t),\ \forall \ell$. As a result, we look for the maximum $p_e$ such that $$f\left(\frac{1}{2\Omega + 1}\sum_{i=-\Omega}^{\Omega}g(\bar{z}^{(\ell-i)}(t);p_e\right) < z^{(\ell)} ~\text{for}~ z^{(\ell)} \in [0,p_e].$$ Let $p_e^*$ and $p_e^\dagger$  denote the maximum success probability for the constrained and unconstrained coupled system, respectively. 
 %and $p_e^\dagger$ represent the same quantity for the unconstrained system.
We will use the analytical approaches recently proposed in \cite{pfister_istc} to find these thresholds. To this end, a potential function is defined  to track the  evolution of the error probability in Eq.~\ref{z_ell}. Let $\textbf{f}(z;p_e): \mb{R}^n \rightarrow \mb{R}^n$ and $\textbf{g}(z): \mb{R}^n \rightarrow \mb{R}^n$ be two component-wise vector functions operating on a vector $\textbf{z}$ such that $[\textbf{f}(\textbf{z};p_e)]_i = f(z_i;p_e)$ and $[\textbf{g}(\textbf{z})]_i = g(z_i)$, where $f(z_i;p_e)$ and $g(z_i)$ are defined  in Lemma~\ref{lem:recursive} .
%recursions (\ref{pi_g_ell}) and (\ref{z_ell_f}). 
Using these definitions, we can rewrite Eq.~\ref{z_ell} in the vector form as \cite{pfister_istc}:
\beq\label{z_vector}
\textbf{z}(t+1) = A^\top\textbf{f}(A\textbf{g}(\textbf{z}(t));p_e)
\eeq
where $A$ is the \emph{coupling matrix} defined as\footnote{Matrix $A$ corresponds to the unconstrained system. A similar matrix can be defined for the constrained case.}:
%\begin{equation*}
%\frac{1}{2\Omega+1}
%\begin{bmatrix}
%\overbrace{\begin{array}{cccc}
%1  &1&  \ldots & 1
%\end{array}
%}^{\Omega} & 0 & 0 & \ldots & 0\\
%\end{bmatrix}
%\end{equation*}
%\vspace{-3.85cm}
\begin{figure}[h!]
\begin{center}
\vspace{-1.85cm}
\begin{tikzpicture}[scale=.5]
%\tikzstyle{every node}=[draw]
%\matrix [draw = white,left delimiter=(,right delimiter=)]
%{
%\draw[help lines] (-5,-3) grid (5,3); 
\node at (-2.9,5.1)[yshift=0,xshift=0,rectangle,minimum size=22mm,below delimiter=\{] (v3) {};
\node at (-2.9,3.4)[rectangle] (v1){$\Omega$};
\node at (-7,0)(v0) {$A=\frac{1}{2\Omega+1}$};
\node at (-2.3,-.3)[rectangle,minimum size=27mm,left delimiter={[}] (v1) {};
\node at (2.9,-.3)[rectangle,minimum size=27mm,right delimiter={]}] (v2) {};
\node at (-4.5,1.8)[rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =5mm,yshift =0mm,rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =12mm,yshift =0mm,rectangle] (v1){$\dots$};
\node at (-4.5,1.8)[xshift =17mm,yshift =0mm,rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =22mm,yshift =0mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =27mm,yshift =0mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =32mm,yshift =0mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =39mm,yshift =0mm,rectangle] (v1){$\dots$};
\node at (-4.5,1.8)[xshift =44mm,yshift =0mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =49mm,yshift =0mm,rectangle] (v1){$0$};

\node at (-4.5,1.8)[xshift =0mm,yshift =-5mm,rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =5mm,yshift =-5mm,rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =12mm,yshift =-5mm,rectangle] (v1){$\dots$};
\node at (-4.5,1.8)[xshift =17mm,yshift =-5mm,rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =22mm,yshift =-5mm,rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =27mm,yshift =-5mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =32mm,yshift =-5mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =39mm,yshift =-5mm,rectangle] (v1){$\dots$};
\node at (-4.5,1.8)[xshift =44mm,yshift =-5mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =49mm,yshift =-5mm,rectangle] (v1){$0$};

\node at (-4.5,1.8)[xshift =0mm,yshift =-9mm,rectangle] (v1){$\vdots$};

\node at (-4.5,1.8)[xshift =0mm,yshift =-16mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =5mm,yshift =-16mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =12mm,yshift =-16mm,rectangle] (v1){$\dots$};
\node at (-4.5,1.8)[xshift =17mm,yshift =-16mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =22mm,yshift =-16mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =27mm,yshift =-16mm,rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =32mm,yshift =-16mm,rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =39mm,yshift =-16mm,rectangle] (v1){$\dots$};
\node at (-4.5,1.8)[xshift =44mm,yshift =-16mm,rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =49mm,yshift =-16mm,rectangle] (v1){$1$};


\node at (-4.5,1.8)[xshift =0mm,yshift =-21mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =5mm,yshift =-21mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =12mm,yshift =-21mm,rectangle] (v1){$\dots$};
\node at (-4.5,1.8)[xshift =17mm,yshift =-21mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =22mm,yshift =-21mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =27mm,yshift =-21mm,rectangle] (v1){$0$};
\node at (-4.5,1.8)[xshift =32mm,yshift =-21mm,rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =39mm,yshift =-21mm,rectangle] (v1){$\dots$};
\node at (-4.5,1.8)[xshift =44mm,yshift =-21mm,rectangle] (v1){$1$};
\node at (-4.5,1.8)[xshift =49mm,yshift =-21mm,rectangle] (v1){$1$};
\end{tikzpicture}
\end{center}
\end{figure}


At this point, the potential function of the unconstrained coupled system could be defined as \cite{pfister_istc}:
\beqa\label{eq:potential}
U(\textbf{z};p_e) &=& \int_{C} \textbf{g}'(\textbf{u})(\textbf{u}-A^\top \textbf{f}(A\textbf{g}(\textbf{u})).d\textbf{u}\nonumber \\
&=& \textbf{g}(\textbf{z})^\top\textbf{z}-G(\textbf{z})-F(A\textbf{g}(\textbf{z});p_e)
\eeqa
where $\textbf{g}'(\textbf{z}) = \hbox{diag}([g'(u_i)])$, $G(\textbf{z}) = \int_{C} \textbf{g}(\textbf{u})\cdot d\textbf{u}$ and $F(\textbf{z}) = \int_{C} \textbf{f}(\textbf{u})\cdot d\textbf{u}$. 

The potential function is defined in the way that $\min\{U(\textbf{z};p_e)\} > 0$ for $p_e < p_e^*$. In contrast, for the unconstrained coupled system, we have $U'(\textbf{z};p_e) > 0$ for $p_e \leq p_e^\dagger$. In other words, in order to find $p_e^*$, it is sufficient to find the maximum $p_e$ such that $\min\{U(\textbf{z};p_e)\} > 0$ \cite{pfister_istc}. We will use this fact and compare the two thresholds later in the simulations section.  Intuitively, we expect to have $p_e^\dagger \leq p_e^*$ (side information only helps), and as a result a better error correction performance for the constrained system.  

The next theorem shows that for $p_e \leq p_e^\dagger$, the error probability of the unconstrained coupled system goes to zero.
\begin{theorem}\label{lemma:unconstrained_coupled}
For $p_e \leq p_e^\dagger$, the fixed point of Eq.~\ref{z_ell} is $0$ and is achieved by iterative updates of Algorithm~\ref{algo:coupled}.
\end{theorem}

Similarly, to address the performance of the constrained coupled system, we  use  the results of \cite{pfister_istc} and \cite{kudekar}.
\begin{theorem}\label{theorem:constrained_coupled}
For the constrained coupled neural associative memory, when $p_e < p_e^*$ the potential function decreases in each iteration. Furthermore, if $L > \Vert U''(\textbf{z};p_e)\Vert_{\infty} / \Delta E(p_e)$, the only fixed point of Eq.~\ref{z_vector} is $\textbf{0}$.
\end{theorem}

\textbf{Pattern retrieval capacity:}
In this part, we prove that the number of patterns that can be memorize by the proposed scheme is exponential in $n$, the pattern size. First, note that this number  is only a function of the size of the subspace that sub-patterns come from. In other words, the number of patterns $\mc{C}$ which the network memorizes does not depend on the learning or recall algorithms (except for its obvious effect on the running time). Therefore, in order to prove that $\mc{C}$ could exponentially scale with $n$, we show that there exists  a subspace with exponentially large number of members (in terms of $n$). The following theorem is the extension of the one we proved in \cite{SK_ISIT2012,KSS_ICML2013} to coupled neural associative networks.

\begin{theorem}\label{theorem_exponential_solution}
Let $\mc{X}$ be the $\mc{C} \times n$ dataset matrix, formed by $\mc{C}$ vectors of length $n$ with entries from the set $\mc{S}$. Let also $k = rn$ for some $0<r<1$. Then, there exists a set of patterns for which $\mc{C} = a^{rn}$, with $a > 1$, and $\hbox{\text{rank}}(\mc{X}) = k <n$.
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Analysis of the Recall Algorithm}
%We start the analysis by considering a theorem in \cite{SK_ISIT2012} stating that Algorithm~\ref{algo:correction} is capable of correcting at least one bit of initial error with high probability.
%\begin{theorem}\label{theorem:isit}\cite{SK_ISIT2012}
%When $\varphi \rightarrow 1$, Algorithm~\ref{algo:correction} can correct a single error in each cluster with probability at least $1- \left(\frac{\bar{d}}{m} \right)^{d_{min}}$, where $\bar{d}$ and $d_{min}$ are the average and minimum degree of the pattern nodes within the cluster domain.
%\end{theorem}
%
%Knowing this fact, let us investigate the error correction algorithm within a single plane. Let $z^{(\ell)}(t)$ denote the \emph{average} probability of error for pattern nodes across neural plane $\ell$ and in iteration $t$. Furthermore, let $\pi^{(\ell)}(t)$ be the \emph{average} probability of a \emph{custer} neuron in plane $\ell$ sending an erroneous message to its neighbors. We will derive recursive expressions for $z^{(\ell)}(t)$ and $\pi^{(\ell)}(t)$. 
%
%A super constraint node in plane $\ell$ receives noisy messages from its neighbors with an average probability of $\bar{z}^{(\ell)}$, where 
%\beq
%\bar{z}^{(\ell)} = \frac{1}{2\Omega+1}\sum_{j=-\Omega}^{\Omega} z^{(\ell-j)}
%\eeq
%with $z^{(i)} = 0$ for $i \leq 0$ and $i > L$. 
%
%Let $\pi_i^{(\ell)}$ denote the the probability that a super constraint node with degree $i$ in plane $\ell$ sends an erroneous message to its neighboring pattern nodes. Then, knowing that each cluster is capable of correcting at least one error, $\pi_i^{(\ell)}$ is equal to the probability of receiving two or more noisy messages from pattern neurons,
%\beq\label{pi_i_ell}
%\pi_i^{(\ell)} = 1-\left(1-\bar{z}^{(\ell)}\right)^{i}-i \bar{z}^{(\ell)} \left(1-\bar{z}^{(\ell)}\right)^{i-1}
%\eeq
%Now, letting $\pi^{(\ell)}(t)$ denote the average probability of sending erroneous nodes by super constraint nodes in plane $\ell$ and in iteration $t$, we will have
%\beqa\label{pi_ell}
%\pi^{(\ell)}(t) &=& \mb{E} \{\pi_i^{(\ell)}\} = \sum_{i} \rho_{i} \pi_i^{(\ell)} \nonumber\\
%&=& 1-\rho(1-\bar{z}^{(\ell)}(t))+\bar{z}^{(\ell)}(t)\rho'(1-\bar{z}^{(\ell)}(t))
%\eeqa
%where $\rho(z) = \sum_i \rho_i z^i$ is the super constraint node degree distribution polynomial and $\rho'(z) = d\rho(z)/dz$. %Note that the above equation is very similar to the peeling decoder recursion in correcting erasures \cite{erasure}, except for the additional $\bar{z}^{(\ell)}(t)\rho'(1-\bar{z}^{(\ell)}(t))$ term which comes from the capability of each cluster to correct one error. 
%
%To simplify notations, let us define the function $g(z)=1-\rho(1-z)+z\rho'(1-z)$ such that
%\beq\label{pi_g_ell}
%\pi^{(\ell)}(t) = g(\bar{z}^{(\ell)}(t))
%\eeq
%
%Now consider a given pattern neuron with degree $j$ in plane $\ell$. In iteration $t+1$, Let $z_j^{(\ell)}(t)$ denote the probability of sending an erroneous message by this node. Then, $z_j^{(\ell)}(t)$ is equal to the probability of this node being noisy in the first place ($p_e$) and having all its super constraint nodes sending erroneous messages in iteration $t$, the average probability of which is $\bar{\pi}^{(\ell)}(t)=\frac{1}{2\Omega + 1}\sum_{i=-\Omega}^{\Omega}\pi^{(\ell-i)}(t)$. Now, since $z^{(\ell)}(t+1) = \mb{E} \{z_j^{(\ell)}(t+1)\}$, we get
%\beqa\label{z_ell}
%z^{(\ell)}(t+1) &=& p_e \sum_j \lambda_j \left( \bar{\pi}^{(\ell)} \right)^{j} \nonumber \\
%%&=& \lambda\left( \bar{\pi}^{(\ell)} \right) \nonumber \\
%&=&p_e \lambda(\bar{\pi}^{(\ell)}) \nonumber \\
%&=& p_e \lambda(\frac{1}{2\Omega + 1}\sum_{i=-\Omega}^{\Omega}g(\bar{z}^{(\ell-i)}(t))
%\eeqa
%
%Again to simplify the notation, let us define the function $f(z;p_e) = p_e \lambda(z)$. This way, we will have the recursion as:
%\beq\label{z_ell_f}
%z^{(\ell)}(t+1) = f(\frac{1}{2\Omega + 1}\sum_{i=-\Omega}^{\Omega}g(\bar{z}^{(\ell-i)}(t);p_e)
%\eeq
%
%Therefore, the decoding operation will be successful if $z^{(\ell)}(t+1) < z^{(\ell)}(t),\ \forall \ell$. As a result, we look for the maximum $p_e$ such that we will have $f(\frac{1}{2\Omega + 1}\sum_{i=-\Omega}^{\Omega}g(\bar{z}^{(\ell-i)}(t);p_e) < z^{(\ell)}$ for $z^{(\ell)} \in [0,p_e]$. Let $p_e^*$ denote this probability for the constrained coupled system and $p_e^\dagger$ represent the same quantity for the unconstrained system.
%
%We will use the analytical approaches recently proposed in \cite{pfister_istc} to derive this threshold. To this end, a potential function is defined ro the system which will be used to track the iterative evolution of the error probability in equation (\ref{z_ell}). Let $\textbf{f}(z;p_e): \mb{R}^n \rightarrow \mb{R}^n$ and $\textbf{g}(z): \mb{R}^n \rightarrow \mb{R}^n$ be two component-wise vector functions operating on a vector $\textbf{z}$ such that $[\textbf{f}(\textbf{z};p_e)]_i = f(z_i;p_e)$ and $[\textbf{g}(\textbf{z})]_i = g(z_i)$, where $f(z_i;p_e)$ and $g(z_i)$ are defined earlier in recursions (\ref{pi_g_ell}) and (\ref{z_ell_f}). Using this defintion, one can rewrite recursion (\ref{z_ell}) in the vector form as \cite{pfister_istc}:
%\beq\label{z_vector}
%\textbf{z}(t+1) = A^\top\textbf{f}(A\textbf{g}(\textbf{z}(t));p_e)
%\eeq
%where $A$ is the \emph{coupling matrix} defined as\footnote{Note that $A$ corresponds to the unconstrained system. A similar matrix can be defined for the constrained case.}:
%\vspace{-1.85cm}
%\begin{center}
%\begin{tikzpicture}[scale=.5]
%%\tikzstyle{every node}=[draw]
%%\matrix [draw = white,left delimiter=(,right delimiter=)]
%%{
%%\draw[help lines] (-5,-3) grid (5,3); 
%\node at (-2.9,5.1)[yshift=0,xshift=0,rectangle,minimum size=22mm,below delimiter=\{] (v3) {};
%\node at (-2.9,3.4)[rectangle] (v1){$\Omega$};
%\node at (-7,0)(v0) {$A=\frac{1}{2\Omega+1}$};
%\node at (-2.3,-.3)[rectangle,minimum size=27mm,left delimiter={[}] (v1) {};
%\node at (2.9,-.3)[rectangle,minimum size=27mm,right delimiter={]}] (v2) {};
%\node at (-4.5,1.8)[rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =5mm,yshift =0mm,rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =12mm,yshift =0mm,rectangle] (v1){$\dots$};
%\node at (-4.5,1.8)[xshift =17mm,yshift =0mm,rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =22mm,yshift =0mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =27mm,yshift =0mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =32mm,yshift =0mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =39mm,yshift =0mm,rectangle] (v1){$\dots$};
%\node at (-4.5,1.8)[xshift =44mm,yshift =0mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =49mm,yshift =0mm,rectangle] (v1){$0$};
%
%\node at (-4.5,1.8)[xshift =0mm,yshift =-5mm,rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =5mm,yshift =-5mm,rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =12mm,yshift =-5mm,rectangle] (v1){$\dots$};
%\node at (-4.5,1.8)[xshift =17mm,yshift =-5mm,rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =22mm,yshift =-5mm,rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =27mm,yshift =-5mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =32mm,yshift =-5mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =39mm,yshift =-5mm,rectangle] (v1){$\dots$};
%\node at (-4.5,1.8)[xshift =44mm,yshift =-5mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =49mm,yshift =-5mm,rectangle] (v1){$0$};
%
%\node at (-4.5,1.8)[xshift =0mm,yshift =-9mm,rectangle] (v1){$\vdots$};
%
%\node at (-4.5,1.8)[xshift =0mm,yshift =-16mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =5mm,yshift =-16mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =12mm,yshift =-16mm,rectangle] (v1){$\dots$};
%\node at (-4.5,1.8)[xshift =17mm,yshift =-16mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =22mm,yshift =-16mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =27mm,yshift =-16mm,rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =32mm,yshift =-16mm,rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =39mm,yshift =-16mm,rectangle] (v1){$\dots$};
%\node at (-4.5,1.8)[xshift =44mm,yshift =-16mm,rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =49mm,yshift =-16mm,rectangle] (v1){$1$};
%
%
%\node at (-4.5,1.8)[xshift =0mm,yshift =-21mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =5mm,yshift =-21mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =12mm,yshift =-21mm,rectangle] (v1){$\dots$};
%\node at (-4.5,1.8)[xshift =17mm,yshift =-21mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =22mm,yshift =-21mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =27mm,yshift =-21mm,rectangle] (v1){$0$};
%\node at (-4.5,1.8)[xshift =32mm,yshift =-21mm,rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =39mm,yshift =-21mm,rectangle] (v1){$\dots$};
%\node at (-4.5,1.8)[xshift =44mm,yshift =-21mm,rectangle] (v1){$1$};
%\node at (-4.5,1.8)[xshift =49mm,yshift =-21mm,rectangle] (v1){$1$};
%\end{tikzpicture}
%\end{center}
%
%
%At this point, the potential function of the unconstrained coupled system could be defined as \cite{pfister_istc}:
%\beqa\label{eq:potential}
%U(\textbf{z};p_e) &=& \int_{C} \textbf{g}'(\textbf{u})(\textbf{u}-A^\top \textbf{f}(A\textbf{g}(\textbf{u})).d\textbf{u}\nonumber \\
%&=& \textbf{g}(\textbf{z})^\top\textbf{z}-G(\textbf{z})-F(A\textbf{g}(\textbf{z});p_e)
%\eeqa
%where $\textbf{g}'(\textbf{z}) = \hbox{diag}([g'(u_i)])$, $G(\textbf{z}) = \int_{C} \textbf{g}(\textbf{u})\cdot d\textbf{u}$ and $F(\textbf{z}) = \int_{C} \textbf{f}(\textbf{u})\cdot d\textbf{u}$.
%
%The potential function is defined in the way that $\min\{U(\textbf{z};p_e)\} > 0$ for $p_e < p_e^*$. For the unonstrained coupled system on the other hand, we have $U'(\textbf{z};p_e) > 0$ for $p_e \leq p_e^\dagger$. In other words, in order to find $p_e^*$, it is sufficient to find the maximum $p_e$ such that $\min\{U(\textbf{z};p_e)\} > 0$ \cite{pfister_istc}. We will use this finding and compare the two thresholds later in the results section but intuitively, one expects that $p_e^\dagger \leq p_e^*$, which means the side information which constrains the coupled system results in better error correction performance.
%
%The next lemma shows that once $p_e \leq p_e^\dagger$, the probability of error in the unconstrained coupled system, shown in equation (\ref{z_ell}), converges to zero.
%\begin{lemma}\label{lemma:unconstrained_coupled}
%For $p_e \leq p_e^\dagger$, the fixed point of equation (\ref{z_ell}) is $0$ and is achieved by iterative updates of Algorithm~\ref{algo:coupled}.
%\end{lemma}
%%\begin{proof}
%%The proof is straightforward and results from the defintion of the potential. Because of the defintion of $p_e^\dagger$, we know that for $p_e \leq p_e^\dagger$ we have $U'(\textbf{z};p_e) > 0$. From equation (\ref{eq:potential}), we have $U'(\textbf{z};p_e) = \textbf{g}'(\textbf{z})(\textbf{z}-A^\top \textbf{f}(A\textbf{g}(\textbf{z}))$. Given that $\textbf{g}'(\textbf{z}) >0$, from $U'(\textbf{z};p_e) > 0$ we conclude that $\textbf{z}-A^\top \textbf{f}(A\textbf{g}(\textbf{z})>0$. This is equivalent to saying that 
%%\bed
%%z^{(\ell)}(t+1) = A^\top \textbf{f}(A\textbf{g}(\textbf{z}^{(\ell)}(t)) < z^{(\ell)}(t).
%%\eed
%%Therefore,$z^{(\ell)}(t)\rightarrow 0,\forall \ell$. 
%%\end{proof}
%
%Now to address the performance of the constrained coupled system, we use the results in \cite{pfister_istc} and \cite{kudekar} to prove the next theorem.
%\begin{theorem}\label{theorem:constrained_coupled}
%For the constrained coupled neural associative memory, when $p_e < p_e^*$ the potential function decreases in each iteration. Furthermore, if $L > \Vert U"(\textbf{z};p_e)\Vert_{\infty} / \Delta E(p_e)$, the only fixed point of the recursion (\ref{z_ell}) is equal to $\textbf{0}$.
%\end{theorem}
%%\begin{proof}
%%The proof of the theorem relies on results from \cite{kudekar} to show that the entries in the vector $\textbf{z}(t) = [z^{(1)}(t),\dots,z^{(L)}(t)]$ are non-decreasing, i.e.  $z^{(1)}(t)\leq z^{(2)}(t)\leq \dots \leq z^{(L)}(t)$. This can be shown using induction and the the functions $\textbf{f}(.,p_e)$ and $\textbf{g}(.)$ are non-decreasing (see the proof of Lemma 22 in \cite{kudekar} for more details).
%%
%%Then, one can apply the result of Lemma 3 in \cite{pfister_istc} to show that the potential function of the constrained coupled system decreases in each iteration. Finally, when $L > \Vert U"(\textbf{z};p_e)\Vert_{\infty} / \Delta E(p_e)$ one could apply Theorem 1 of \cite{pfister_istc} to show the convergence of the probability of errors to zero.
%%\end{proof}
%



